Hunt for new phenomena using large jet multiplicities and missing transverse momentum with ATLAS in 4.7 fb^-1 of sqrt(s) = 7 TeV proton-proton collisions

Results are presented of a search for new particles decaying to large numbers of jets in association with missing transverse momentum, using 4.7 fb^-1 of pp collision data at sqrt(s) = 7 TeV collected by the ATLAS experiment at the Large Hadron Collider in 2011. The event selection requires missing transverse momentum, no isolated electrons or muons, and from >=6 to >=9 jets. No evidence is found for physics beyond the Standard Model. The results are interpreted in the context of a MSUGRA/CMSSM supersymmetric model, where, for large universal scalar mass m_0, gluino masses smaller than 840 GeV are excluded at the 95% confidence level, extending previously published limits. Within a simplified model containing only a gluino octet and a neutralino, gluino masses smaller than 870 GeV are similarly excluded for neutralino masses below 100 GeV.

==> frontmatter.tex <==
\RequirePackage{lineno}
\newcommand*\patchAmsMathEnvironmentForLineno[1]{%
  \expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
  \expandafter\let\csname oldend#1\expandafter\endcsname\csname end#1\endcsname
  \renewenvironment{#1}%
     {\linenomath\csname old#1\endcsname}%
     {\csname oldend#1\endcsname\endlinenomath}}%
\newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
  \patchAmsMathEnvironmentForLineno{#1}%
  \patchAmsMathEnvironmentForLineno{#1*}}%
\AtBeginDocument{%
\patchBothAmsMathEnvironmentsForLineno{equation}%
%\patchBothAmsMathEnvironmentsForLineno{equation*}%
\patchBothAmsMathEnvironmentsForLineno{align}%
\patchBothAmsMathEnvironmentsForLineno{flalign}%
\patchBothAmsMathEnvironmentsForLineno{alignat}%
\patchBothAmsMathEnvironmentsForLineno{gather}%
\patchBothAmsMathEnvironmentsForLineno{multline}%
}
\usepackage{atlasphysics}
\usepackage[bf,tight]{subfigure}
\usepackage{mathrsfs}
\usepackage{graphicx}
\usepackage{multirow}
\usepackage{rotating}
\usepackage{slashed}
% \usepackage{mcite}
\usepackage{amsmath}
\usepackage{url}
\usepackage{textpos}
\usepackage{placeins}
%\usepackage{atlascover}

\usepackage{hyperref}
%\usepackage{hypernat}  % makes hyperref work with natbib

%\biboptions{sort,merge}

\input{susydefs}
\graphicspath{./figures/}
\DeclareGraphicsExtensions{.pdf}

\newcommand{\mSUGRA}{MSUGRA/CMSSM}
\newcommand{\mSUGRAShortened}{CMSSM}
\newcommand{\ourpt}{p_\mathrm{T}}
\newcommand{\mT}{\ensuremath{m_{\rm T}}}
\newcommand{\anactualptmissvecwithapinit}{{\vec{p}}_\mathrm{T}^\mathrm{\,miss}}
\newcommand{\ourvecptmiss}{\ensuremath{\anactualptmissvecwithapinit}}
\newcommand{\ourmagptmiss}{{\ensuremath \MET}}
\renewcommand{\HT}{{\ensuremath{H_{\rm T}}}}
\newcommand{\metsig}{{\ensuremath{\ourmagptmiss/\sqrt{\HT}}}}
\newcommand{\rootgev}{{\ensuremath{\GeV^{1/2}}}}
\newcommand{\pthreshold}{{\ensuremath{p_{<}}}}
\newcommand{\mult}{{\ensuremath{n_{\rm jet}}}}
\newcommand{\paper}{paper}
\newcommand{\sigmamaxbsm}{\ensuremath{\sigma_{\rm BSM,max}^{95\%}}}
\newcommand{\nmaxbsm}{\ensuremath{N_{\rm BSM,max}^{95\%}}}
\newcommand{\smin}{{\ensuremath{s_\textrm{min}}}}
\newcommand{\smax}{{\ensuremath{s_\textrm{max}}}}
\newcommand{\alpgen}{{\tt Alpgen}}
\newcommand{\herwig}{{\tt Herwig}}
\newcommand{\sherpa}{{\tt Sherpa}}
\newcommand{\jimmy}{{\tt Jimmy}}
\newcommand{\prospino}{{\tt Prospino}}
\newcommand{\cteqVER}[1]{{\tt CTEQ#1}}
\newcommand{\mstwVER}[1]{{\tt MSTW#1}}
\newcommand{\nnpdfVER}[1]{{\tt NNPDF#1}}
\newcommand{\nllfastVER}[1]{{\tt NLL-fast#1}}
\newcommand{\alpgenVER}[1]{{\tt Alpgen#1}}
\newcommand{\prospinoVER}[1]{{\tt Prospino#1}}
\newcommand{\herwigppVER}[1]{{\tt Herwig++#1}}
\newcommand{\isajetVER}[1]{{\tt ISAJET++#1}}
\newcommand{\msugra}{MSUGRA/CMSSM}
\newcommand{\leptonic}{`leptonic'}
\newcommand{\Leptonic}{`Leptonic'}
\newcommand{\citemsugraandcmssm}{\cite{Chamseddine:1982jx,Barbieri:1982eh,Ibanez:1982ee,Hall:1983iz,Ohta:1982wn,Kane:1993td}}
\newcommand{\oursubref}[1]{{\bf (\subref{#1})}}
\newcommand{\ourtabref}[1]{Table~\ref{#1}}
\newcommand{\ourfigref}[1]{Figure~\ref{#1}}
\newcommand{\oursecref}[1]{Section~\ref{#1}}
\newcommand{\comment}[1]{{\em[#1]}}



==> susydefs.tex <==

\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\figsref}[1]{Figures.~\ref{#1}}
%\newcommand{\partref}[1]{part~\ref{#1}}
\newcommand{\Secref}[1]{Section~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}

% susy-specific variables
\newcommand{\meff}{\ensuremath{m_{\mathrm{eff}}}} % This was an M, but all our other m's are in lower case and M_eff sticks out like a sore thumb.  So I've changed it to something more relaxing.
\newcommand{\mt}{\ensuremath{m_\mathrm{T}}}
\newcommand{\mttwo}{\ensuremath{m_\mathrm{T2}}}
\newcommand{\mc}{\ensuremath{m_\mathrm{C}}}
\newcommand{\mct}{\ensuremath{m_\mathrm{CT}}}
%\newcommand{\alphat}{\ensuremath{\ensuremath{\alpha_{T}}}}
%\newcommand{\etmiss}{\ensuremath{\slashed{E}_T}}
%\newcommand{\pmiss}{\ensuremath{\slashed{p}}}
%\newcommand{\ptmiss}{\ensuremath{\slashed{p}_T}}
%\newcommand{\Ptmiss}{\ensuremath{{\slashed{\bf p}}_T}}
\def\Ptmiss{\ensuremath{\vec{E}_\mathrm{T}^{\mathrm{miss}}}}

\def\lsim{\mathrel{\rlap{\lower4pt\hbox{\hskip1pt$\sim$}}
    \raise1pt\hbox{$<$}}}                % less than or approx. symbol
\def\gsim{\mathrel{\rlap{\lower4pt\hbox{\hskip1pt$\sim$}}
    \raise1pt\hbox{$>$}}}                % greater than or approx. symbol

%\renewcommand{\thesubfigure}{\alpha{subfigure}}
\makeatletter
\renewcommand{\p@subfigure}{\arabic{figure}}
\renewcommand{\thesubfigure}{\alph{subfigure}}
\renewcommand{\@thesubfigure}{(\thesubfigure)}
\makeatother

